Mechanism Design for Subadditive Agents via an Ex-Ante Relaxation

We consider the problem of maximizing revenue for a monopolist offering multiple items to multiple heterogeneous buyers. We develop a simple mechanism that obtains a constant factor approximation under the assumption that the buyers' values are additive subject to a feasibility constraint and independent across items. Importantly, different buyers in our setting can have different constraints on the sets of items they desire. Our mechanism is a sequential variant of two-part tariffs. Prior to our work, simple approximation mechanisms for such multi-buyer problems were known only for the special cases of all unit-demand or all additive value buyers. Our work expands upon and unifies long lines of work on unit-demand settings and additive settings. We employ the ex ante relaxation approach developed by Alaei (2011) for reducing a multiple-buyer mechanism design problem with an ex post supply constraint into single-buyer ones with ex ante supply constraints. Solving the single-agent problems requires us to significantly extend techniques developed in the context of additive values by Li and Yao (2013) and their extension to subadditive values by Rubinstein and Weinberg (2015).

==> bottomstuff.tex <==
\begin{bottomstuff}
This work is supported by the National Science Foundation, grant CCF-1101429 and
grant CCF-1320854.

Authors' addresses: S. Chawla and J. B. Miller, Department of Computer Sciences,
University of Wisconsin--Madison; email: \{shuchi,bmiller\}@cs.wisc.edu
\end{bottomstuff}


==> prophet.tex <==
\section{Single-Agent Approximation for General Matroids}
\label{sec:general-matroid}

The proof of Lemma~\ref{lem:approx-partition} relied upon the existence of a
threshold-based prophet inequality for partition matroids, which translates
directly into a pricing scheme. No such prophet inequality is known for general
matroids, but a recent result of \citet{fsz-15} provides a
\scnote{demand-limiting pricing scheme}.

\begin{theorem}
%\label{thm:ocrs}
 (\cite{fsz-15}) For a general matroid $\feas$, constant $b \in (0,1)$, \exante\
 constraints $\eaprobs \in b\ptope$, and corresponding \exante\ prices
 $\eaprices$, there exists a submatroid $\feas' \subseteq \feas$ such that
 \[\eaprices\cdot\eaprobs \leq \frac{1}{1-b}\easrev(\dists,\feas').\]
 Furthermore, the prices and constraint $\feas'$ which achieve this bound are
 efficiently approximable.
 %\scnote{I
 %believe this is true, and would reduce the constant from 4 to 2 in our case
 %because we are already assuming $\eaprobs \in 1/2\ptope$. Need to write up the
 %argument. If true, we would need the other results only for computational
 %efficiency.}
\end{theorem}

Combining Theorems~\ref{thm:single-agent} and \ref{thm:ocrs}, we obtain
Lemma~\ref{lem:approx-general} for general matroids.

\begin{lemma}[\bf Single-agent approximation \# 2]
\label{lem:approx-general}
  Let $\dist$ be any value distribution and $\feas$ be an arbitrary
  matroid with feasible polytope $\ptope$. Then, for any $\eaprob\in
  \frac 12\ptope$, there exists a submatroid $\feas'\subseteq\feas$,
  such that 
\[ \earev(\dist, \feas) \le 33.1 \eatrev(\dist, \feas') \]
\end{lemma}

%\begin{theorem}
%\label{thm:graphic-matroid}
% (\cite{CHMS-STOC10}) For a graphic matroid $\feas$, \exante\ constraints
% $\eaprobs$, and corresponding \exante\ prices $\eaprices$, there exists
% $\feas' \subseteq \feas$ such that
% \[\eaprices\cdot\eaprobs \leq 3\easrev(\dists,\feas').\]
%\end{theorem}

